An Empirical Exploration of Deep Recurrent Connections and Memory Cells Using Neuro-Evolution

Neuro-evolution and neural architecture search algorithms have gained increasing interest due to the challenges involved in designing optimal artificial neural networks (ANNs). While these algorithms have been shown to possess the potential to outperform the best human crafted architectures, a less common use of them is as a tool for analysis of ANN structural components and connectivity structures. In this work, we focus on this particular use-case to develop a rigorous examination and comparison framework for analyzing recurrent neural networks (RNNs) applied to time series prediction using the novel neuro-evolutionary process known as Evolutionary eXploration of Augmenting Memory Models (EXAMM). Specifically, we use our EXAMM-based analysis to investigate the capabilities of recurrent memory cells and the generalization ability afforded by various complex recurrent connectivity patterns that span one or more steps in time, i.e., deep recurrent connections. EXAMM, in this study, was used to train over 10.56 million RNNs in 5,280 repeated experiments with varying components. While many modern, often hand-crafted RNNs rely on complex memory cells (which have internal recurrent connections that only span a single time step) operating under the assumption that these sufficiently latch information and handle long term dependencies, our results show that networks evolved with deep recurrent connections perform significantly better than those without. More importantly, in some cases, the best performing RNNs consisted of only simple neurons and deep time skip connections, without any memory cells. These results strongly suggest that utilizing deep time skip connections in RNNs for time series data prediction not only deserves further, dedicated study, but also demonstrate the potential of neuro-evolution as a means to better study, understand, and train effective RNNs.

==> 04-examm.tex <==
\section{Evolutionary eXploration of Augmenting Memory Models}
\label{sec:examm}

The EXAMM algorithm presented in this work expands on an earlier algorithms, EXALT~\cite{desell2015evolving} which can evolve RNNs with either simple neurons or LSTM cells and EXACT which evolves convolutional neural networks for image classification~\cite{desell2017arxiv,desell2018accelerating}. It further refines EXALT's mutation operations to reduce hyperparameters using statistical information from parental RNN genomes. Also, EXALT only used a single steady state population, and EXAMM expands on this to use islands, which have been shown by Alba and Tomassini to greatly improve performance of distributed evolutionary algorithms, potentially providing superlinear speedup~\cite{alba2002parallelism}. A master process maintains each population of islands, and generates new RNNs from islands in a round robin manner to be trained upon request by workers. When a worker completes training a RNN, it is inserted into the island it was generated from if its fitness (mean squared error on the test data) is better than the worst in the island, and then the worst RNN in the island is removed. This asynchrony is particularly important as the generated RNNs will have different architectures, each taking a different amount of time to train. By having a master process control the population, workers can complete the training of the generated RNNs at whatever speed they can and the algorithm is naturally load balanced. This allows EXAMM to scale to the number of available processors, having a population size independent of processor availability, unlike synchronous parallel evolutionary strategies. The EXAMM codebase has a multithreaded implementation for multicore CPUs as well as an MPI~\cite{mpif94mpi} implementation for use on high performance computing resources.

\subsection{Mutation and Recombination Operations}
\label{sec:mutation}

RNNs are evolved with edge-level operations, as done in NEAT, as well as with new high level node mutations as in EXALT and EXACT. Whereas NEAT only requires innovation numbers for new edges, EXAMM requires innovation numbers for both new nodes, new edges and new recurrent edges. The master process keeps track of all node, edge and recurrent edge innovations made, which are required to perform the crossover operation in linear time without a graph matching algorithm.  Figures~\ref{fig:edge_mutations} and~\ref{fig:node_mutations_1} display a visual walkthrough of all the mutation operations used by EXAMM. Nodes and edges selected to be modified are highlighted, and then new elements to the RNN are shown in green. Edge innovation numbers are not shown for clarity. Enabled edges are in black, disabled edges are in grey.

It should be noted that for the following operations, whenever an edge is added, unless otherwise specified, it is probabilistically selected to be a recurrent connection with the following recurrent probability: $p = \frac{n_{re}}{n_{ff} + n_{re}}$, where $n_{re}$ is the number of enabled recurrent edges and $n_{ff}$ is the number of enabled feed forward edges in the parent RNN.  A recurrent connection will go back a randomly selected number of time steps with bound specified as search parameters (in this work, 1 to 10 time steps), allowing for recurrent connections of varying time spans.  Any newly created node is selected uniformly at random as a simple neuron or from the memory cell types specified by the EXAMM run input parameters.

\begin{figure}
    \centering
    \subfloat[The edge between Input 1 and Output 1 is selected to be split. A new node with innovation number (IN) 1 is created. ]{
        \includegraphics[width=0.45\textwidth]{figures/01_split_edge.png}
    }\hfill
    \subfloat[Input 3 and Node IN 1 are selected to have an edge between them added.]{
        \includegraphics[width=0.45\textwidth]{figures/02_add_edge.png}
    }

    \subfloat[The edge between Input 3 and Output 1 is enabled.]{
        \includegraphics[width=0.45\textwidth]{figures/03_enable_edge.png}
    }\hfill
    \subfloat[A recurrent edge is added between Output 1 and Node IN 1]{
        \includegraphics[width=0.45\textwidth]{figures/04_add_recurrent_edge.png}
    }

    \subfloat[The edge between Input 3 and Output 1 is disabled.]{
        \includegraphics[width=0.45\textwidth]{figures/05_disable_edge.png}
    }
    \caption{\label{fig:edge_mutations} Edge mutation operations.}
\end{figure}



\subsubsection{Edge Mutations:}
\label{sec:edge_mutations}

\paragraph{Disable Edge} This operation randomly selects an enabled edge or recurrent edge in a RNN genome and disables it so that it is not used.  The edge remains in the genome. As the \emph{disable edge} operation can potentially make an output node unreachable, after all mutation operations have been performed to generate a child RNN genome, if any output node is unreachable that RNN genome is discarded without training.

\paragraph{Enable Edge} If there are any disabled edges or recurrent edges in the RNN genome, this operation selects a disabled edge or recurrent edge at random and enables it.

\paragraph{Split Edge} This operation selects an enabled edge at random and disables it. It creates a new node and two new edges, and connects the input node of the split edge to the new node, and the new node to the output node of the split edge. If the split edge was recurrent, the new edges will also be recurrent (with the same time skip); otherwise they will be feed forward.

\paragraph{Add Edge} This operation selects two nodes $n_1$ and $n_2$ within the RNN Genome at random, such that $depth_{n_1} < depth_{n_2}$ and such that there is not already an edge between those nodes in this RNN Genome. Then it adds an edge from $n_1$ to $n_2$. 

\paragraph{Add Recurrent Edge} This operation selects two nodes $n_1$ and $n_2$ within the RNN Genome at random and then adds a recurrent edge from $n_1$ to $n_2$, selecting a time span as described before. The same two nodes can be connected with multiple recurrent connections, each spanning different times; however it will not create a duplicate recurrent connection with the same time span.

\subsubsection{Node Mutations:}
\label{sec:node_mutations}
    
\begin{figure}
    \centering
    \subfloat[A node with IN 2 is selected to be added at a depth between the inputs \& Node IN 1. Edges are randomly added to Input 2 and 3, and Node IN 1 and Output 1.]{
        \includegraphics[width=0.45\textwidth]{figures/06_add_node.png}
    }

    \subfloat[Node IN 1 is selected to be split. It is disabled with its input/output edges. It is split into Nodes IN 3 and 4, which get half the inputs. Both have an output edge to Output 1 since there was only one output from Node IN 1.]{
        \includegraphics[width=0.45\textwidth]{figures/07_split_node.png} 
    }

    \subfloat[Node IN 2 and 3 are selected for a merger (input/output edges are disabled). Node IN 5 is created with edges between all their inputs/outputs.]{
        \includegraphics[width=0.45\textwidth]{figures/08_merge_node.png}
    }
    \caption{\label{fig:node_mutations_1} Node mutation operations.}
\end{figure}

\begin{figure}
    \ContinuedFloat
    \centering
    \subfloat[Node IN 1 is selected to be enabled, along with all its input and output edges.]{
        \includegraphics[width=0.45\textwidth]{figures/09_enable_node.png}
    }

    \subfloat[Node IN 5 is selected to be disabled, along with all its input and output edges.]{
        \includegraphics[width=0.45\textwidth]{figures/10_disable_node.png}
    }

    \caption{\label{fig:node_mutations_2} Node mutation operations (continued).}
\end{figure}


\paragraph{Disable Node} This operation selects a random non-output node and disables it along with all of its incoming and outgoing edges. Note that this allows for input nodes to be dropped out, which can be useful when it is not previously known which input parameters are correlated to the output.

\paragraph{Enable Node} This operation selects a random disabled node and enables it along with all of its incoming and outgoing edges.

\paragraph{Add Node} This operation selects a random depth between 0 and 1, noninclusive. Given that the input node is always depth 0 and the output nodes are always depth 1, this depth will split the RNN in two. A new node is created at that depth, and the number of input and output edges and recurrent edges are generated using normal distributions with mean and variances equal to the mean and variances for the input/output edges and recurrent edges of all nodes in the parent RNN.  

\paragraph{Split Node} This operation takes one non-input, non-output node at random and splits it. This node is disabled (as in the disable node operation) and two new nodes are created at the same depth as their parent. At least one input and one output edge are assigned to each of the new nodes, of a duplicate type from the parent, with the others being assigned randomly, ensuring that the newly created nodes have both inputs and outputs. 

\paragraph{Merge Node} This operation takes two non-input, non-output nodes at random and combines them.  Selected nodes are disabled (as in the disable node operation) and a new node is created at depth equal to the average of its parents. This node is connected to the inputs and outputs of its parents with a duplicate type from the parent; as input edges connected to lower depth nodes and output edges connect to greater depth nodes. 

\subsubsection{Other Operations:}

%\paragraph{Crossover} utilizes two hyperparameters, the \emph{more fit crossover rate} and the \emph{less fit crossover rate}. Two parent RNN genomes are selected, and the child RNN genome is generated from every edge that appears in both parents. Edges that only appear in the more fit parent are added randomly at the \emph{more fit crossover rate}, and edges that only appear in the less fit parent are added randomly at the \emph{less fit crossover rate}. Edges not added by either parent are also carried over into the child RNN genome, however they are set to disabled. Nodes are then added for each input and output of an edge.  If the more fit parent has a node with the same innovation number, it is added from the more fit parent. 

\paragraph{Crossover} creates a child RNN using all reachable nodes and edges from two parents. A node or edge is reachable if there is a path of enabled nodes and edges from an input node to it as well as a path of enabled nodes and edges from it to an output node, \ie, a node or edge is reachable if it actually affects the RNN. Crossover can be done either within an island (\emph{intra-island}) or between islands (\emph{inter-island}). Inter-island crossover selects a random parent in the target island, and the best RNN from the other islands.

\paragraph{Clone} creates a copy of the parent genome, initialized to the same weights.  This allows a particular genome to continue training in cases where further training may be more beneficial than performing a mutation or crossover.


\subsection{Lamarckian Weight Initialization}
\label{sec:lamarckian_weight_initialization}

For RNNs generated during population initialization, the weights are initialized uniformly at random between $-0.5$ and $0.5$. Biases and weights for new nodes and edges are initialized from a normal distribution based on the average, $\mu$, and variance, $\sigma^2$, of the parents' weights. However, RNNs generated through mutation or crossover re-use parental weights, allowing the RNNs to train from where the parents are left off, \ie, \emph{``Lamarckian'' weight initialization}.

During crossover, in the case where an edge or node exists in both parents, the child weights are generated by recombining the parents' weights.  Given a random number $-0.5 <= r <= 1.5$, a child's weight $w_c$ is set to $w_c = r(w_{p2} - w_{p1}) + w_{p1}$, where $w_{p1}$ is the weight from the more fit parent, and $w_{p2}$ is the weight from the less fit parent. This allows the child weights to be set along a gradient calculated from the weights of the two parents.

This weight initialization strategy is particularly important as newly generated RNNs do not need to be completely retrained from scratch. In fact, the RNNs only need to be trained for a few epochs to investigate the benefits of newly added structures.  In this work, the generated RNNs are only trained for 10 epochs (see Section~\ref{sec:experimental_design}), where training a static RNN structure from scratch may require hundreds or even thousands of epochs.


\subsection{A Collection of Memory Cells}
\label{sec:mem_models}
Node types vary in terms of complexity and with their design governing the form of the underlying memory structure. Simple neurons can be evolved into generalized versions of traditional Elman and Jordan neurons as EXAMM adds recurent connections. Below describes how simple neurons can evolve to generalized Elman and Jordan neurons, as well as one complex cell, the Delta-RNN. The Appendix describes all of the cell structures incorporated into EXAMM's cell library, including the minimally gated unit (MGU) \cite{zhou2016minimal}, the update-gated RNN (UGRNN) \cite{collins2016capacity}, the Gated Recurrent Unit (GRU) \cite{chung2014empirical}, and Long Short Term Memory (LSTM) \cite{hochreiter1997long}. %These cell models together make up the internal library accessible to EXAMM for possible selection during its metaheuristic search. 



\noindent
\textbf{Elman, Jordan and Arbitrary Recurrent Connections:} 
In EXAMM, simple neurons are represented as traditional neurons with potentially both recurrent and feed forward inputs. $I$ is the set of all nodes with a feed forward connection to simple neuron $j$ while $R$ is the set of all nodes with a recurrent connection to simple neuron $j$. At time step $t$, the output is a weighted summation of all feed forward inputs, where $w_{ij}$ is the feed forward weight connecting node $i$ to node $j$, plus a weighted summation of recurrent inputs, where $v_{rjk}$ is the recurrent weight from node $r$ at time step $t-k$ to the node $j$, where $k$ is the time span of the recurrent connection. Thus the state function $s$ for a computing a simple neuron is:\footnote{The bias is omitted for clarity and simplicity of presentation.}
\vspace{-2mm}
\begin{align*}
    s_j(t) &= \phi_s \bigg( \sum_{i \in I} w_{ij} \cdot s_i(t) + \sum_{r \in R,k} v_{rjk} \cdot s_r(t-k) \bigg)
\vspace{-22mm}
\end{align*}
The overall state is a linear combination of the projected input and an affine transformation of the vector summary of the past. The post-activation function, $\phi_s(\cdot)$, can be any differentiable element-wise function, however for the purposes of this work it was limited to the hyperbolic tangent, $\phi(v) = tanh(v) = (e^{(2v)} - 1) / (e^{(2v)} + 1)$. %Future work will involve selection of a set of activation functions including the logistic sigmoid and linear rectifier.

%The post-activation function $\phi_s(\cdot)$ can be any differentiable element-wise function, such as the logistic sigmoid $\phi_s(v) = \sigma(v) = 1/(1 + e^{-v})$, the hyperbolic tangent $\phi(v) = tanh(v) = (e^{(2v)} - 1) / (e^{(2v)} + 1)$, or the linear rectifier $\phi_s(v) = relu(v) = max(0, v)$. Note that we recover the pure simple neuron by simply setting and fixing $v_{ij} = 0$, which is also one possible node that EXAMM may select during the search process.

%EXAMM also evolves a form of recurrent node inspired by the Jordan RNN \cite{jordan1997serial}, which, in the original model, uses output-to-state recurrent connections instead of state-to-state connections connections to compute its internal state. In EXAMM, this is generalized by allowing nodes to feature cross-layer recurrent connections, \ie, the node is not restricted to only be connected itself but also to connect to a node at any other depth. Recurrent connections in Jordan/Elman RNNs traditionally only span one time step, however EXAMM generalizes this as well to allow connections spanning time steps between user-specified markers (in this case 1 \& 10).

Elman-RNNs~\cite{elman1990finding} connect recurrent nodes to themselves and potentailly all other hidden nodes in the same layer. Jordan-RNNs \cite{jordan1997serial} have recurrent connections from output node(s) to hidden node(s). EXAMM can evolve Elman connections when the \emph{add recurrent edge} mutation adds a recurrent edge from a simple neuron back to itself, and Jordan connections when it adds a recurrent edge from an output to a simple neuron. It generalizes these structures by allowing varying time spans (Jordan and Elmann network traditionally span only one time step) and arbitrary recurrent connections between from any pair of simple neurons or cells.

\noindent
\textbf{The Delta RNN ($\Delta$-RNN) Cell:} 
For models more complex than the simple RNN model, we looked to derive a vast set of gated neural architectures unified under a recent framework known as the Differential State Framework (DSF) \cite{ororbia2017diff}. A DSF neural model is essentially a composition of an inner function used to compute state proposals and an outer ``mixing'' function used to decide how much of a state proposal is incorporated into a slower moving state, \ie, the longer term memory. These models are better equipped to handle the vanishing gradient problem induced by the difficulty of learning long-term dependencies over sequences \cite{bengio1994learning}. Other models that can be derived under the DSF include the LSTM, the GRU, and the MGU \cite{ororbia2017diff}. One of the simplest DSF models is the $\Delta$-RNN, which has been shown to perform competitively with more complex memory models in problems ranging from language modeling \cite{ororbia2017diff,ororbia2018using} to image decoding \cite{ororbia2018learned}. With $\{\alpha,\beta_1,\beta_2,b_j,m\}$ as learnable coefficient scalars, the $\Delta$-RNN state is defined as:
%\vspace{-2mm}
\begin{align*}
e^{w}_j &= \sum_{i \in I} w_{ij} \cdot s_i(t) + \sum_{r \in R,k} v_{rjk} \cdot s_r(t-k),\quad e^{v}_j = m \cdot s_j(t-1) \\
d^1_j &= \alpha \cdot e^{v}_j \cdot e^{w}_j,\quad d^2_j = \beta_1 \cdot e^{v}_j + \beta_2 \cdot e^{w}_j, \quad r_j = \sigma(e^{w}_j + b_j) \\
\widetilde{s}_j(t) &= \phi_s(d^1_j + d^2_j), \quad s_j(t) = \Phi_s( (1 - r_j) \cdot \widetilde{s}_j(t) + r_j \cdot s_j(t-1) \\
\vspace{-10mm}
\end{align*}


